Implementation and validation of the FRi3D flux rope model in EUHFORIA

The Flux Rope in 3D (FRi3D, Isavnin, 2016), a coronal mass ejection (CME) model with global three-dimensional (3D) geometry, has been implemented in the space weather forecasting tool EUHFORIA (Pomoell and Poedts, 2018). By incorporating this advanced flux rope model in EUHFORIA, we aim to improve the modelling of CME flank encounters and, most importantly, the magnetic field predictions at Earth. After using synthetic events to showcase FRi3D's capabilities of modelling CME flanks, we optimize the model to run robust simulations of real events and test its predictive capabilities. We perform observation-based modelling of the halo CME event that erupted on 12 July 2012. The geometrical input parameters are constrained using the forward modelling tool included in FRi3D with additional flux rope geometry flexibilities as compared to the pre-existing models. The magnetic field input parameters are derived using the differential evolution algorithm to fit FRi3D parameters to the in situ data at 1 AU. An observation-based approach to constrain the density of CMEs is adopted, in order to achieve a better estimation of mass corresponding to the FRi3D geometry. The CME is evolved in EUHFORIA's heliospheric domain and a comparison of FRi3D's predictive performance with the previously implemented spheromak CME in EUHFORIA is presented. For this event, FRi3D improves the modelling of the total magnetic field magnitude and Bz at Earth by ~30% and ~70%, respectively. Moreover, we compute the expected geoeffectiveness of the storm at Earth using an empirical Dst model and find that the FRi3D model improves the predictions of minimum Dst by ~20% as compared to the spheromak CME model. Finally, we discuss the limitations of the current implementation of FRi3D in EUHFORIA and propose possible improvements.

==> references.tex <==
@article{Winslow_2021,
	doi = {10.3847/1538-4357/ac0439},
	url = {https://doi.org/10.3847/1538-4357/ac0439},
	year = 2021,
	month = {jul},
	publisher = {American Astronomical Society},
	volume = {916},
	number = {1},
	pages = {40},
	author = {Reka M. Winslow and Camilla Scolini and No{\'{e}} Lugaz and Antoinette B. Galvin},
	title = {The Effect of Stream Interaction Regions on {ICME} Structures Observed in Longitudinal Conjunction},
	journal = {The Astrophysical Journal},
	abstract = {We study two interplanetary coronal mass ejections (ICMEs) observed at Mercury and at 1 au by spacecraft in longitudinal conjunction, investigating the question: what causes the drastic alterations observed in some ICMEs during propagation, while other ICMEs remain relatively unchanged? Of the two ICMEs, the first one propagated relatively self-similarly, while the second one underwent significant changes in its properties. We focus on the presence or absence of large-scale corotating structures in the ICME propagation space between Mercury and 1 au, which have been shown to influence the orientation of ICME magnetic structures and the properties of ICME sheaths. We determine the flux rope orientation at the two locations using force-free flux rope fits as well as the classification by Nieves-Chinchilla et al. We also use measurements of plasma properties at 1 au, the size evolution of the sheaths and magnetic ejecta with heliocentric distance, and identification of structures in the propagation space based on in situ data, remote-sensing observations, and simulations of the steady-state solar wind to complement our analysis. Results indicate that the changes observed in one ICME were likely caused by a stream interaction region, while the ICME exhibiting little change did not interact with any transients between Mercury and 1 au. This work provides an example of how interactions with corotating structures in the solar wind can induce fundamental changes in ICMEs. Our findings can help lay the foundation for improved predictions of ICME properties at 1 au.}
}


@article{https://doi.org/10.1002/2015JA022307,
author = {Winslow, Reka M. and Lugaz, Noé and Schwadron, Nathan A. and Farrugia, Charles J. and Yu, Wenyuan and Raines, Jim M. and Mays, M. Leila and Galvin, Antoinette B. and Zurbuchen, Thomas H.},
title = {Longitudinal conjunction between MESSENGER and STEREO A: Development of ICME complexity through stream interactions},
journal = {Journal of Geophysical Research: Space Physics},
volume = {121},
number = {7},
pages = {6092-6106},
keywords = {ICME, HPS, HCS, magnetic topology},
doi = {https://doi.org/10.1002/2015JA022307},
url = {https://agupubs.onlinelibrary.wiley.com/doi/abs/10.1002/2015JA022307},
eprint = {https://agupubs.onlinelibrary.wiley.com/doi/pdf/10.1002/2015JA022307},
abstract = {Abstract We use data on an interplanetary coronal mass ejection (ICME) seen by MErcury Surface, Space ENvironment, GEochemistry, and Ranging (MESSENGER) and STEREO A starting on 29 December 2011 in a near-perfect longitudinal conjunction (within 3°) to illustrate changes in its structure via interaction with the solar wind in less than 0.6 AU. From force-free field modeling we infer that the orientation of the underlying flux rope has undergone a rotation of ∼80° in latitude and ∼65° in longitude. Based on both spacecraft measurements as well as ENLIL model simulations of the steady state solar wind, we find that interaction involving magnetic reconnection with corotating structures in the solar wind dramatically alters the ICME magnetic field. In particular, we observed a highly turbulent region with distinct properties within the flux rope at STEREO A, not observed at MESSENGER, which we attribute to interaction between the ICME and a heliospheric plasma sheet/current sheet during propagation. Our case study is a concrete example of a sequence of events that can increase the complexity of ICMEs with heliocentric distance even in the inner heliosphere. The results highlight the need for large-scale statistical studies of ICME events observed in conjunction at different heliocentric distances to determine how frequently significant changes in flux rope orientation occur during propagation. These results also have significant implications for space weather forecasting and should serve as a caution on using very distant observations to predict the geoeffectiveness of large interplanetary transients.},
year = {2016}
}

